Comparing Stochastic Differential Equations and Agent-Based Modelling and Simulation for Early-stage Cancer

There is great potential to be explored regarding the use of agent-based modelling and simulation as an alternative paradigm to investigate early-stage cancer interactions with the immune system. It does not suffer from some limitations of ordinary differential equation models, such as the lack of stochasticity, representation of individual behaviours rather than aggregates and individual memory. In this paper we investigate the potential contribution of agent-based modelling and simulation when contrasted with stochastic versions of ODE models using early-stage cancer examples. We seek answers to the following questions: (1) Does this new stochastic formulation produce similar results to the agent-based version? (2) Can these methods be used interchangeably? (3) Do agent-based models outcomes reveal any benefit when compared to the Gillespie results? To answer these research questions we investigate three well-established mathematical models describing interactions between tumour cells and immune elements. These case studies were re-conceptualised under an agent-based perspective and also converted to the Gillespie algorithm formulation. Our interest in this work, therefore, is to establish a methodological discussion regarding the usability of different simulation approaches, rather than provide further biological insights into the investigated case studies. Our results show that it is possible to obtain equivalent models that implement the same mechanisms; however, the incapacity of the Gillespie algorithm to retain individual memory of past events affects the similarity of some results. Furthermore, the emergent behaviour of ABMS produces extra patters of behaviour in the system, which was not obtained by the Gillespie algorithm.

==> FiguresAndTables.tex <==
%% Figures                       %%

\section*{Figures}

\subsection*{Figure 1 - Tumour cell agent}

\begin{figure}[h]
% \begin{center}
  \resizebox{3.8cm}{!}{\includegraphics{./Figure1_AgentOne.eps}}
% \end{center}
% \caption{Tumour cell agent}
 \caption{}
 \label{fig:AgentOne}
\end{figure}


\subsection*{Figure 2 - ABMS state charts for case 1}
   \begin{figure}[!htpb]
%\centering
\subfigure[Tumour cell agent]{
   \includegraphics[scale =0.56] {Figure2a_TumourAgent.eps}
 }
\qquad
 \subfigure[Effector cell agent]{
   \includegraphics[scale =0.56] {Figure2b_EffectorAgents.eps}
 }
 %\caption{ABMS state charts for case 1}
 \caption{}
 \label{fig:CaseStudy2:ABS}
\end{figure}

\newpage
\subsection*{Figure 3 - Results for case 1 scenario 1}

\begin{figure}[!htpb]
%\centering
\subfigure{
   \includegraphics[scale =0.5] {Figure3a_Scenario1SD.eps}
 }
\qquad
 \subfigure{
   \includegraphics[scale =0.5] {Figure3b_Scenario1ABS.eps}

 }
 \caption{}
 \label{fig:CaseStudy2:Case1:ResultsScenario1}
%\caption{Results for scenario 1}
\end{figure}


\subsection*{Figure 4 - Results for case 1 scenario 2}

\begin{figure}[!htpb]
%\centering
\subfigure{
   \includegraphics[scale =0.5] {Figure4a_Scenario2SD.eps}
 }
\qquad
 \subfigure{
   \includegraphics[scale =0.5] {Figure4b_Scenario2ABS.eps}

 }
\caption{}
\label{fig:CaseStudy2:Case1:ResultsScenario2}
%\caption{Results for scenario 2}
\end{figure}

\newpage
\subsection*{Figure 5 - Results for case 1 scenario 3}

\begin{figure}[!htpb]
%\centering
\subfigure{
   \includegraphics[scale =0.5] {Figure5a_Scenario3SD.eps}
 }
\qquad
 \subfigure{
   \includegraphics[scale =0.5] {Figure5b_Scenario3ABS.eps}

 }
 \caption{}
 \label{fig:CaseStudy2:Case1:ResultsScenario3}
%\caption{Results for scenario 3}
\end{figure}



\subsection*{Figure 6 - Results for case 1 scenario 4}

\begin{figure}[!htpb]
%\centering
\subfigure{
   \includegraphics[scale =0.5] {Figure6a_Scenario4SD.eps}
 }
\qquad
 \subfigure{
   \includegraphics[scale =0.5] {Figure6b_Scenario4ABS.eps}

 }
 \caption{}
 \label{fig:CaseStudy2:Case1:ResultsScenario4}
%\caption{Results for scenario 4}
\end{figure}

\newpage
\subsection*{Figure 7 - ABMS state charts for the agents of case 2}

\begin{figure}[!htpb]
  \resizebox{16cm}{!}{\includegraphics{Figure7_ABSModelCase2.eps}}
 \caption{}
 \label{fig:ABSModelThreeEquation}
\end{figure}


\subsection*{Figure 8 - ODEs and ABMS results for effector cells of case 2}
\begin{figure}[!htpb]
\subfigure{
   \includegraphics[scale =0.5] {Figure8a_EffectorSD1.eps}
 }
\qquad
 \subfigure{
   \includegraphics[scale =0.5] {Figure8b_EffectorABS1.eps}
 }
\caption{}
\label{fig:CaseStudy2:Case2Effector}
\end{figure}

\newpage
\subsection*{Figure 9 - ODEs and ABMS results for tumour cells of case 2}
\begin{figure}[htpb]
\centering
\subfigure{
   \includegraphics[scale =0.5] {Figure9a_TumourSD1.eps}
 }
\qquad
 \subfigure{
   \includegraphics[scale =0.5] {Figure9b_TumourABS1.eps}
 }
\caption{}
\label{fig:CaseStudy2:Case2Tumour}
\end{figure}


\subsection*{Figure 10 - ODEs and ABMS results for IL2 of case 2}
\begin{figure}[!htbp]
\subfigure{
   \includegraphics[scale =0.5] {Figure10a_IL2SD1.eps}
 }
\qquad
 \subfigure{
   \includegraphics[scale =0.5] {Figure10b_IL2ABS1.eps}
 }
\caption{}
\label{fig:CaseStudy2:Case2IL2}
\end{figure}

\newpage
\subsection*{Figure 11 - ABS state charts for the agents of case 3}
\begin{figure}[!htpb]
  \resizebox{16cm}{!}{\includegraphics{Figure11_ABSModel.eps}}
\caption{}
\label{fig:ABSModelFourEquation}
\end{figure}


\subsection*{Figure 12 - ODEs and ten runs of ABMS results for effector cells of case 3}

\begin{figure}[!htpb]
\subfigure{
   \includegraphics[scale =0.5] {Figure12a_EffectorSD.eps}
 }
\qquad
 \subfigure{
   \includegraphics[scale =0.5] {Figure12b_EffectorABS10.eps}
 }
\caption{}
\label{fig:CaseStudy2:Case3Effector}
\end{figure}

\newpage

\subsection*{Figure 13 - ODEs and ten runs of ABMS results for tumour cells of case 3}
\begin{figure}[ht]
\subfigure{
   \includegraphics[scale =0.5] {Figure13a_TumourSD.eps}
 }
\qquad
 \subfigure{
   \includegraphics[scale =0.5] {Figure13b_TumourABS10.eps}
 }
\caption{}
\label{fig:CaseStudy2:Case3Tumour}
\end{figure}


\subsection*{Figure 14 - ODEs and ten runs of ABMS results for IL-2 of case 3}
\begin{figure}[!htpb]
\subfigure{
   \includegraphics[scale =0.5] {Figure14a_IL2SD.eps}
 }
\qquad
 \subfigure{
   \includegraphics[scale =0.5] {Figure14b_IL2ABS10.eps}
 }
\caption{}
\label{fig:CaseStudy2:Case3IL2}
\end{figure}

\newpage
\subsection*{Figure 15 - ODEs and ten runs of ABMS results for TGF-$\beta$ of case 3}

\begin{figure}[!h]
\subfigure{
   \includegraphics[scale =0.5] {Figure15a_TGFSD.eps}
 }
\qquad
 \subfigure{
   \includegraphics[scale =0.5] {Figure15b_TGFABS.eps}
 }
\caption{}
\label{fig:CaseStudy2:Case3TGF}
\end{figure}


\subsection*{Figure 16 - ODEs and ABMS results for effector cells of case 3}

\begin{figure}[!htpb]
\subfigure{
   \includegraphics[scale =0.5] {Figure12a_EffectorSD.eps}
 }
\qquad
 \subfigure{
   \includegraphics[scale =0.5] {Figure16b_EffectorABS.eps}
 }
\caption{}
\label{fig:CaseStudy2:Case3Effector2}
\end{figure}

\newpage
\subsection*{Figure 17 - ODEs and ABMS results for tumour cells of case 3}

\begin{figure}[!htpb]
\subfigure{\includegraphics[scale =0.5] {Figure13a_TumourSD.eps}}
\qquad
 \subfigure{
   \includegraphics[scale =0.5] {Figure17b_TumourABS.eps}
 }
\caption{}
\label{fig:CaseStudy2:Case3Tumour2}
\end{figure}


\subsection*{Figure 18 - ODEs and ABMS results for IL-2 of case 3}
\begin{figure}[!htpb]
\subfigure{
   \includegraphics[scale =0.5] {Figure14a_IL2SD.eps}
 }
\qquad
 \subfigure{
   \includegraphics[scale =0.5] {Figure18b_IL2ABS.eps}
 }
\caption{}
\label{fig:CaseStudy2:Case3IL22}
\end{figure}
\newpage
\subsection*{Figure 19 - ODEs and ABMS results for TGF-$\beta$ of case 3}
\begin{figure}[!htpb]
\subfigure{
   \includegraphics[scale =0.5] {Figure15a_TGFSD.eps}
 }
\qquad
 \subfigure{
   \includegraphics[scale =0.5] {Figure15b_TGFABS.eps}
 }
\caption{}
\label{fig:CaseStudy2:Case3TGF2}
\end{figure}


%% Tables                        %%


\section*{Tables}

\subsection*{Table 1 - Case studies considered}

\begin{table}[!hb]
%\centering
\caption{}
\begin{tabular}{|l|c|c|c|}
\hline
Case Study                             & Number of populations             & Population size  & Complexity \\
\hline
\hline
1) Tumour/Effector                     & 2                                 &  5 to 600        &  Low       \\
\hline
2) Tumour/Efector/IL-2                 & 3                                 & $10^4$           &  Medium    \\
\hline
3) Tumour/Effector/IL-2/ TGF-$\beta$   & 4                                 &  $10^4$          &  High       \\
\hline
\end{tabular}
\label{Tab:CaseStudies}
\end{table}

\subsection*{Table 2 - Agents' parameters and behaviours for the tumour growth model}

\begin{table}[ht]
%\caption{Agents' parameters and behaviours for the tumour growth model}
%\begin{center}
\caption{}
\begin{tabular}{|l|l|l|}
\hline
Parameters                     &  Reactive behaviour   & Proactive behaviour       \\
\hline \hline

$a$, $alpha$, $b$ and $beta$   & Dies if $rate < 0$    & Proliferates if $rate > 0$                \\
\hline
\end{tabular}
\label{Tab:TumourGrowthBehaviours}
%\end{center}
\end{table}

\newpage
\subsection*{Table 3 - Agents' parameters and behaviours for case 1}

\begin{table}[!htpb]
%\caption{Agents' parameters and behaviours for case 1}
%\begin{center}
\caption{}
\begin{tabular}{|l|l|l|l|}
\hline
Agent          & Parameters              &  Reactive behaviour       & Proactive behaviour                \\
\hline \hline
\multirow{4}{*}
{Tumour Cell}  & $a$ and $b$             & Dies (with age)                     &  \\
               \cline{2-4}
               & $a$ and $b$             &                           & Proliferates              \\
               \cline{2-4}
               & $m$                     &                           & Damages effector cells\\
               \cline{2-4}
               & $n$                     &  Dies killed by effector cells &                 \\
\hline
\hline
\multirow{4}{*}
{Effector Cell}& $m$                     &  Dies (with age)            & \\
               \cline{2-4}
               & $d$                     &  Dies per apoptosis            & \\
               \cline{2-4}
               & $p$ and $g$             &                           & Proliferates             \\
               \cline{2-4}
               & $s$                     &  Is injected as treatment &\\
\hline
\end{tabular}
\label{Tab:CaseStudy2:Case1:AgentsBehaviours}
%\end{center}
\end{table}



\subsection*{Table 4 - Transition rates calculations from the mathematical equations for case 1}

\begin{table}[!htpb]
%\begin{center}
\caption{}
\begin{tabular}{|l|l|l|l|}
\hline
Agent                &  Transition              & Mathematical equation                               & Transition rate       \\
\hline \hline
\multirow{12}{*}
{Tumour Cell}        &&&\\
                     &  proliferation           & $aT(1 - Tb)$                                        & $a - (TotalTumour.b)$   \\
                     &&&\\
                     \cline{2-4}
                     &&&\\
                     &  death                   & $aT(1 - Tb)$                                        & $a - (TotalTumour.b)$   \\
                     &&&\\
                     \cline{2-4}
                     &&&\\
                     &  dieKilledByEffectorCells& $nTE$                                               & $n.TotalEffectorCells$\\
                     &&&\\
                     \cline{2-4}
                     &&&\\
                     &  causeEffectorDamage     & $mTE$                                               & $m$\\
                     &&&\\

\hline
\hline
\multirow{8}{*}
{Effector Cell}      &&&\\

                     & Proliferation            & $\frac{pTE}{g+T}$ & $\frac{p. TotalTumourCells}{g+TotalTumourCells}$\\
                     &&&\\
                     \cline{2-4}
                     &&&\\
                     & DieWithAge               & $dE$                      & $d$\\
                     &&&\\
                     \cline{2-4}
                     &&&\\
                     & DiePerApoptosis          & $mTE$                     & message from tumour   \\
\hline
\end{tabular}
\label{Tab:TumourEffectorTransitionRatesCalculations1}
%\end{center}
\end{table}

\newpage
\subsection*{Table 5 - Simulation parameters for different scenarios of case 1. For the other parameters, the values are the same in all experiments, i.e. $a=1.636$, $g=20.19$, $m=0.00311$, $n=1$ and $p=1.131$.}

\begin{table}[!htpb]
\caption{}
\begin{tabular}{|l|c|c|c|}
\hline
Scenario  & b     &  d     & s      \\
\hline \hline
1         &0.002 & 0.1908  & 0.318  \\
\hline
2         &0.004 & 2       & 0.318  \\
\hline
3         &0.002 & 0.3743  & 0.1181 \\
\hline
4         &0.002 & 0.3743  & 0  \\
\hline
\end{tabular}
\label{Tab:CaseStudy2:TumourEffectorsParameters}
%\caption{Simulation parameters for different scenarios. For the other parameters, the values are the same in all experiments, i.e. $a=1.636$, $g=20.19$, $m=0.00311$, $n=1$ and $p=1.131$.}
\end{table}


\subsection*{Table 6 - Wilcoxon test with $5\%$ significance level comparing case 1 simulation results}

\begin{table}[!htpb]
%\caption{Wilcoxon test comparing case 1 simulation results}

%  \centering
\caption{}
  \begin{tabular}{|l|l|c|c|c|c|}
  \hline
  Implementation    & Cells                   &  \multicolumn{4}{c|}{Scenario (p-value)}  \\
                           &                  &  1 &  2 & 3 &  4 \\

  \hline
  \hline
  {\em ABS}          & {\it Tumour}           & 0      &  0      &  0.8591 &  0        \\
                     & {\it Effector}         & 0.3789 &  0.6475 &  0      &  0        \\
\hline
  {\em ABS - Fix 1}  & {\it Tumour}           & 0      &  0      &  0      &  0.0011   \\
                     & {\it Effector}         & 0      &  0.3023 &  0      &  0        \\
\hline
  {\em ABS - Fix 2}  & {\it Tumour}           & 0      &  0      &  0      &  0        \\
                     & {\it Effector}         & 0      &  0      &  0      &  0        \\

 \hline
  \end{tabular}
\label{tab:CaseStudy2:Case1:Wilcoxon}
\end{table}

\subsection*{Table 7 - Agents' parameters and behaviours for case 2}

\begin{table}[h]
\caption{}
%\caption{Agents' parameters and behaviours for case 2}
\begin{tabular}{|l|l|l|l|}
\hline
Agent          & Parameters             & Reactive behaviour            &  Proactive behaviour            \\
\hline \hline
\multirow{6}{*}
{Effector Cell}& $mu2$                  & Dies                       & \\
               \cline{2-4}
               & $p1$ and $g1$          &                            & Reproduces                      \\
               \cline{2-4}
               & $c$                    & Is recruited               &                                 \\
               \cline{2-4}
               & $s1$                   & Is injected as treatment   &                                 \\
               \cline{2-4}
               & $p2$ and $g3$          &                            & Produces IL-2\\
               \cline{2-4}
               & $aa$ and $g2$          &                            & Kills tumour cells\\

\hline
\hline
\multirow{4}{*}
{Tumour Cell}  & $a$ and $b$            &  Dies  & \\
               \cline{2-4}
               & $a$ and $b$            &                             & Proliferates         \\
               \cline{2-4}
               & $aa$ and $g2$          &  Dies killed by effector cells&                      \\
               \cline{2-4}
               & $c$                    &                               & Induces effector recruitment\\
\hline
\hline
\multirow{3}{*}
{IL-2}         &  $p2$ and $g3$         &  Is produced   &\\
               \cline{2-4}
               &  $mu3$                 &  Is lost       &\\
               \cline{2-4}
               &  $s2$                  &  Is injected   &\\

\hline
\end{tabular}
\label{Tab:ABSModelThreeEquation}
\end{table}

\newpage
\subsection*{Table 8 - Transition rates calculations from the mathematical equations for case 2}

\begin{table}[ht]
\caption{}
\begin{tabular}{|l|l|l|l|}
\hline
Agent                &  Transition              & Mathematical equation             & Transition rate       \\
\hline \hline
\multirow{12}{*}
{Effector Cell}      &&&\\
                     & Reproduce                & $\frac{p_1.I_LE}{g1+IL\_2}$        & $\frac{p_1.TotalIL\_2.TotalEffector}{g1+TotalIL\_2}$\\
                     &&&\\
                     \cline{2-4}
                     &&&\\
                     & Die                      & $\mu_2E$                           & $mu2$\\
                     &&&\\
                     \cline{2-4}
                     &&&\\
                     & killTumour               & $\frac{a_aET}{g2 + T}$             & $aa \frac{TotalTumour}{g2 + TotalTumour}$\\
                     &&&\\
                     \cline{2-4}
                     &&&\\
                     & ProduceIL2               &$\frac{p2ET}{g3 + T}$               & $\frac{p2.TotalTumour}{g3 + TotalTumour}$\\
                     &&&\\

\hline
\hline

\multirow{8}{*}
{Tumour Cell}         &  Reproduce               & $aT(1 - bT)$                        & $a - (TotalTumour.b)$   \\
                     &&&\\
                     \cline{2-4}
                     &&&\\
                     &  Die                     & $aT(1 - bT)$                        & $a - (TotalTumour.b)$ \\
                     &&&\\
                     \cline{2-4}
                     &&&\\
                     &  DieKilledByEffector     & $\frac{a_aTE}{g2+T}$                & message from effector\\
                     &&&\\

\hline
\hline

IL-2                & Loss                      & $\mu_3I_L$                             & $mu3$\\
\hline
\end{tabular}
\label{Tab:TumourEffectorTransitionRatesCalculations}
\end{table}

\subsection*{Table 9 - Parameter values for case 2}

\begin{table}[ht!]
\caption{}
\begin{tabular}{|l|l|}
\hline
Parameter & Value\\
\hline
\hline
a         & 0.18\\
\hline
b & 0.000000001\\
\hline
c & 0.05\\
\hline
aa & 1\\
\hline
g2 & 100000\\
\hline
s1 & 0\\
\hline
s2 & 0 \\
\hline
mu2 & 0.03\\
\hline
p1 & 0.1245\\
\hline
g1 & 20000000\\
\hline
p2 & 5\\
\hline
g3 & 1000\\
\hline
mu3 & 10\\
\hline
\end{tabular}
 \label{Tab:CaseStudy2:ParametersModelCase2}
\end{table}

\newpage

\subsection*{Table 10 - Wilcoxon test with $5\%$ significance level comparing the results from the ODEs and ABMS for case 2}

\begin{table}[!htpb]
\caption{}
\begin{tabular}{|l|c|}
\hline
Population                  & p \\
\hline
\hline
Effector                    &  0.7231  \\
\hline
Tumour                      &  0.5710  \\
\hline
IL2                         &  0.4711  \\
\hline
\end{tabular}
 \label{Tab:Mode3EquationsWilcoxon}
\end{table}

\subsection*{Table 11 - Agents' parameters and behaviours for case 3}

\begin{table}[!htpb]
\caption{}
\begin{tabular}{|l|l|l|l|}
\hline
Agent          & Parameters                    & Reactive behaviour            &  Proactive behaviour            \\
\hline \hline
\multirow{4}{*}
{Effector Cell}& $mu1$                         & Dies                       & \\
               \cline{2-4}
               & $p1$, $g1$, $q1$ and $q2$     &                            & Reproduces                      \\
               \cline{2-4}
               & $c$                           & Is recruited               &                                 \\
               \cline{2-4}
               & $aa$ and $g2$                 &                            & Kills tumour cells\\

\hline
\hline
\multirow{6}{*}
{Tumour Cell}  & $a$                           &  Dies  & \\
               \cline{2-4}
               & $a$                           &                             & Proliferates         \\
               \cline{2-4}
               & $aa$ and $g2$                 &  Dies killed by effector cells&                      \\
               \cline{2-4}
               & $g3$ and $p2$                 &  Has growth stimulated       &\\
               \cline{2-4}
               & $p4$ and $tetha$              &                              & Produces TGF-$\beta$\\
               \cline{2-4}
               & $c$                           &                              & Induces effector recruitment\\
\hline
\hline
\multirow{2}{*}
{IL-2}          &  $alpha$, $p3$ and $g4$       &  Is produced   &\\
                \cline{2-4}
                &  $mu2$                        &  Is lost       &\\
\hline
\multirow{3}{*}
{TGF-$\beta$}  &  $p4$ and $tetha$             & Is produced &\\
               \cline{2-4}
               &  $mu3$                        & Is lost & \\
               \cline{2-4}
               &  $p2$ and $g3$                &         & Stimulates tumour growth\\

\hline
\end{tabular}
\label{Tab:ABSModelFourEquation}
\end{table}

\newpage
\subsection*{Table 12 - Transition rates calculations from the mathematical equations for case 3}

\begin{table}[!ht]
\caption{}
\begin{tabular}{|l|l|l|l|}
\hline
Agent                &  Transition           & Mathematical equation                                         & Transition rate       \\
\hline \hline
\multirow{12}{*}
{Effector Cell}      & \multirow{3}{*}{Reproduce} & $\frac{p_1IE}{g1+I}\times$    & $\frac{p_1\times TotalIL\_2}{g1+TotalIL\_2}\times$\\

                     &                          &$\left ( p1 - \frac{q1S}{q2 + S} \right )$ & $\left ( p1 - \frac{q1 \times TotalTGFBeta}{q2 + TotalTGFBeta} \right )$\\

                     \cline{2-4}
                     &&&\\
                     & Die                       & $\mu_1E$                      & $mu1$\\
                     &&&\\

                     \cline{2-4}

                     &&&\\
                     & ProduceIL2                & $\frac{p3TE}{(g4 + T)(1+alphaS)}$         & $\frac{p3.TotalTumour}{(g4 + TotalTumour)(1+alpha.TotalTGF)}$\\
                     &&&\\
                     \cline{2-4}
                     &&&\\
                     & KillTumour                & $\frac{a_aTE}{g2+T}$  & $\frac{aa \times TotalTumour \times TotalEffector}{g2+TotalTumour}$\\

                     &&&\\

\hline
\hline
&&&\\
\multirow{15}{*}
{Tumour Cell}        &  Reproduce            & $\left ( aT \left (1- \frac{T}{1000000000}\right ) \right )$  & $\left ( TotalTumour.a \left( 1- \frac{TotalTumour}{1000000000}\right ) \right )$\\
                     &&&\\
                     \cline{2-4}
                     &&&\\

                     &  Die                  & $\left ( aT \left (1- \frac{T}{1000000000}\right ) \right )$  & $\left ( TotalTumour.a \left( 1- \frac{TotalTumour}{1000000000}\right ) \right )$\\
                     &&&\\
                     \cline{2-4}
                     &&&\\

                     &  DieKilledByEffector  & $\frac{a_a.TE}{g2+T}$              & message from effector\\
&&&\\
\cline{2-4}
                     &&&\\

                     & ProduceTGF & $\frac{p4T^2}{teta^2 + T^2}$                  & $\frac{p4.TumourCells}{teta^2 + TumourCells^2}$\\
                     &&&\\
                     \cline{2-4}
                     &&&\\
                     & EffectorRecruitment & $\frac{cT}{1 + \gamma S}$             & $\frac{c}{1 + gamma.TotaltGF}$\\
&&&\\
\hline
\hline
&&&\\
IL-2                & Loss                   & $\mu_2I$                             & $mu2$\\
&&&\\
\hline
\hline
&&&\\
\multirow{4}{*}
{TGF-$\beta$}         & Loss                   & $\mu_3S$                           & $mu3$\\
                    &&&\\
                    \cline{2-4}
                     & stimulates &&\\
                     &TumourGrowth             & $\frac{p2T}{g3+S}$                  & $\frac{p2.TotalTGF}{g3 + TotalTGF}$\\
&&&\\
\hline
\end{tabular}
\label{Tab:TumourEffector4TransitionRatesCalculations}
\end{table}

\newpage

\subsection*{Table 13 - Parameter values for case 3}
\begin{table}[!htpb]
\caption{}
\begin{tabular}{|l|l|}
\hline
Parameter & Value\\
\hline
\hline
a         & 0.18\\
\hline
aa & 1\\
\hline
alpha     & 0.001\\
\hline
c & 0.035\\
\hline
g1 & 20000000\\
\hline
g2 & 100000\\
\hline
g3 & 20000000\\
\hline
g4 & 1000\\
\hline
gamma & 10\\
\hline
mu1 & 0.03 \\
\hline
mu2 & 10\\
\hline
mu3 & 10\\
\hline
p1 & 0.1245\\
\hline
p2 & 0.27\\
\hline
p3 & 5\\
\hline
p4 & 2.84\\
\hline
q1 & 10\\
\hline
q2 & 0.1121\\
\hline
theta & 1000000\\
\hline
k & 10000000000\\
\hline
\end{tabular}
 \label{Tab:CaseStudy2:ParametersModelCase3}
\end{table}


\subsection*{Table 14 - Summary of findings}


\begin{table}[!ht]
\caption{}
%\caption{Summary of findings}
\footnotesize
\begin{tabular}{|l | l | l | c | c |c|}
\hline
Case Study          & Outcome of the  comparison             &  Explanation                    & Population size\\
\hline
\hline
                    &                                        & $\bullet$ It appears that variabilities       & Varied from         \\
1) Tumour/Effector  & $\bullet$ Most results were different  &   in small populations have major        &  5 to 600           \\
                    &                                        &  impacts in the outcomes &                     \\
\hline
                    &                                        &  $\bullet$ Large populations    &                       \\
2) Tumour/Efector   & $\bullet$ Results were statistically
/IL-2                      the same                               &  $\bullet$ Less variability in  & $10^4$        \\
                    &                                        & the agents' populations         &                     \\
\hline
                    & $\bullet$Different runs with outcome
                      variations                             & $\bullet$ Agent-based
                                                               stochasticity                   &         \\
                    & $\bullet$ Simulations produced
                      alternative scenarios                  &  $\bullet$ New scenarios need further &    \\
3) Tumour/Effector/ & $\bullet$The behaviour of the curves   &  investigations to assess       &  $10^4$             \\
IL-2/ TGF-$\beta$   & is less erratic for agents             &  their feasibility              &                     \\
                    &                                        &  $\bullet$ Large numbers of agents &                  \\

\hline
\end{tabular}
\label{Tab:Findings}
\end{table}


==> Intro.tex <==
\section{Introduction}

Advances in cancer immunology have been facilitated  by the joint work of immunologists and mathematicians~\cite{Wodarz:2002,Eftimie2010,Gruber:2003}.  Some of the knowledge regarding interactions between the immune system and tumours is a result of using mathematical models.  Most existing mathematical models in cancer immunology are based on sets of ordinary differential equations (ODEs)~\cite{Eftimie2010}. This approach, however, has limitations pertaining problems involving spatial interactions  or emerging properties~\cite{Borshchev:2004,Louzoun:2007}. In addition, the analysis of ODE models is conducted at a high level of aggregation of the system entities. An alternative to ODE modelling that overcomes these limitations is systems simulation modelling.  It is a set of methodologies and applications which mimic the behaviour of a real system~\cite{Pidd:2003,Robinson:2004,Banks:2009}. Systems simulation modelling has also benefits compared to real world experimentation in immunology, including time and cost effectiveness due to the resource-intensiveness of the biological environment. Furthermore, in a simulation environment it is possible to systematically generate different scenarios and conduct experiments. In addition, the ``what-if'' scenarios studied in such an environment do not require ethics approval.

Agent-based modelling and simulation (ABMS) is an object-oriented system modelling and simulation approach that employs autonomous entities that interact with each other~\cite{Macal:2005,Wooldridge:2002,Macal:2010b}. The focus during the modelling process is on defining templates for the individual entities (agents) being modelled and defining possible interactions between these entities. The agent behaviour is described by rules that determine how these entities learn, adapt and interact with each other. The overall system behaviour arises from the agents’ individual behaviour and their interactions with other agents and the environment. For cancer immunology, it can amalgamate in vitro data on individual interactions between cells and molecules of the immune system and tumour cells to build an overview of the system as a whole~\cite{Kim:2009}. Few studies, however, apply ABMS to cancer research. Although there are examples showing the success of simulation aiding advances in immunology~\cite{Look:1981,Zand:2004,Figge:2005,Casal:2005,Segovia-Juarez:2004,Nuno:2007}, this set of methodologies is still not popular. There are several reasons for this: (1) ABMS is not well known in the immunology research field; (2) although simulation is acknowledged as being a useful tool by immunologists, there is no knowledge of how to use it; and (3) there is not enough trust in the results produced by simulation.

Our aim is to outline the potential contribution of ABMS to help cancer-related immune studies. In order to achieve our aim, we use a case study approach. We have chosen three well-established mathematical models describing interactions between the immune system and early-stage cancer as our test candidates. These models consist of systems of ODEs solved numerically for a time interval. By studying these models we focus on the following three research enquiries:

\begin{enumerate}
   \item Is it possible to obtain an equivalent ABMS model based on the mathematical equations from the ODEs (i.e. can we create an object oriented model by re-using ODEs that have been created for modelling behaviour at an aggregate level)?
   \item Do we get equivalent simulation outputs for both approaches?
   \item What benefits could we gain by re-conceptualizing a mathematical model under an ABMS view?
\end{enumerate}


\subsection*{Case studies}

The case studies are chosen by considering aspects such as the population size, modelling effort, model complexity, observation of the ODEs outcome results and the  number of different populations modelled. The mathematical models chosen vary largely within these aspects and therefore we can perform a more robust analysis of our experiments, as shown in Table~\ref{Tab:CaseStudies}.

The first case study considered is based on an ODE model involving interactions between tumour cells and generic effector cells. The second case study adds to the previous model the influence of IL-2 cytokine molecules in the immune responses of effector cells towards tumour cells. The final case study comprises an ODE model of interactions between effector cells, tumour cells, and IL-2 and TGF-$\beta$ molecules. For all case studies, the mathematical model as well as the ABMS model are presented, the outcomes are contrasted and the benefits of each approach are assessed. The models differ in terms of complexity of interactions, population sizes and the number of agents involved in the interactions (Table~\ref{Tab:CaseStudies}).

The remainder of this paper is organized as follows. We start with a literature review of works comparing ODEs and ABMS for different simulation domains. First, we show general work that has been carried out and then we focus on research concerned with the comparison for immunological problems.  Finally, we discuss gaps in the literature regarding cancer research. In the methodology section, we introduce our agent-based modelling development process and the methods used for conducting the experimentation. In the following section, we present our case studies, comparison results and discussions. In the last section, we finally draw our overall conclusions and outline future research opportunities.


==> Methodology.tex <==
\section*{Methodology}
\label{Methodology}

In this section we outline the activities and methods necessary to realise our objectives. We examine case studies of established mathematical models that describe some immune cells and molecules interacting with tumour cells. These case studies were chosen by considering aspects such as the behaviour of the entities of the model, size (and number) of populations involved and the modelling effort. The original mathematical models are built under an agent-based approach and results compared.

ABMS is capable of representing space; however, as we chose mathematical models which do not consider spatial interactions, our corresponding ABMS models do not regard space (distance) and how it would affect the simulation outcomes. The outcome samples obtained by ODEs and ABMS were statistically compared using the Wilcoxon rank-sum test to formally establish whether they are statistically different from each other. This test is applied as it is robust when the populations are not normally distributed; this is the case for the samples obtained by the ODEs and ABMS. Other approaches for assessing whether the two samples are statistically different, such as the t-test, could provide inaccurate results as they perform poorly when the samples are non-normal.

\subsection*{The agent-based model development}

The agent-based models were implemented using ($AnyLogic^{TM}$ 6.5~\cite{AnyLogic:2010}). For the agent design we follow the steps defined in~\cite{Figueredo:2011}: (1) identify the agents (cells and molecules), (2) define their behaviour (die, kill tumour cells, suffer apoptosis), (3) add them to an environment,  and (4) establish connections to finally run the simulations, as further discussed next:

{\bf 1. Identify the possible agents}. For this purpose, we use some characteristics defined in~\cite{Macal:2005}. An agent is: (1) self-contained, modular, and a uniquely identifiable individual; (2) autonomous and self-directed; (3) a construct with states that varies over time; and (4) social, having dynamic interactions with other agents that impact its behaviour. By looking at the ODE equations, therefore, the variables that are differentiated over time (their disaggregation) will either be corresponding to agents or states of one agent~\cite{Figueredo:2010,Figueredo:2011}. The decision whether the stock is an agent or an agent state varies depending on the problem investigated. Based on our case studies, however, we suggest that: (1) these variables preferably become states when they represent accumulations of elements from the same population; or (2) they become agents when they represent accumulations from different populations. For example, if you have an ODE $\frac{dx}{dt} = y$, $x$ should either be an agent or an agent state, depending on the problem context.

{\bf 2. Identify the behaviour and rules of each agent}. In our case, the agent's behaviours will be determined by mathematical equations converted into rules. Each agent has two different types of behaviours: reactive and proactive behaviours. The reactive behaviour occurs when the agents perceive the context in which they operate and react to it appropriately. The proactive behaviour describes the situations when the agent has the initiative to identify and solve an issue in the system.

{\bf 3. Implement the agents}. Based on step 2 we develop the agents. The agents are defined by using state charts diagrams from the unified modelling language (UML)~\cite{CCI:2005-23}. With state charts it is possible to define and visualize the agents' states, transitions between the states, events that trigger transitions, timing and agent actions~\cite{Borshchev:2004}. Moreover, at this stage, the behaviours of each agent are implemented using the simulation tool. Most of our transitions occur according to a certain rate. For our implementation, the rate is obtained from the mathematical equations.

{\bf 4. Build the simulation}. After agents are defined, their environment and behaviour previously established should be incorporated in the simulation implementation. Moreover, in this step we include parameters and events that control the agents or the overall simulation.

For example, let us consider a classical ODE which describes an early-stage tumour growth pattern~\cite{Eftimie2010}:

\begin{equation}
\label{Eq:GeneralTumourGrowth}
 \frac{dT}{dt} = Tf(T)
\end{equation}

where:

\begin{itemize}
\item $T$ is the tumour cell population at time $t$,
\item $T(0) > 0$,
\item $f(T)$ specifies the density dependence in proliferation
and death of the tumour cells. The density dependence factor can
be written as:
\end{itemize}

\begin{equation}
f(T) = p(T) - d(T)
\end{equation}

where:

\begin{itemize}
\item $p(T)$ defines tumour cells proliferation
\item $d(T)$ define tumour cells death
\end{itemize}

The expressions for $p(T)$ and $d(T)$ are generally defined by
power laws:

\begin{equation}
p(T) = aT^\alpha \label{SubEq:p(T)}
\end{equation}

\begin{equation}
 d(T)=bT^\beta
\label{SubEq:d(T)}
\end{equation}

In this case, our agent would be a tumour cell that replicates and dies according to the parameters $\alpha$ and $\beta$. The tumour cell agent behaviours are ``proliferate'' or ``die'', according to the rate defined by the mathematical model. If the rate is positive, there is proliferation, otherwise, death occurs (Table~\ref{Tab:TumourGrowthBehaviours}).

The tumour cell assumes two states, alive and dead, as shown in Figure~\ref{fig:AgentOne}. In the alive state, these cells can replicate and die. If the growth rate is positive, the cell replicates according to the rate value; otherwise, it dies. There is, therefore a branch connecting the two transitions $proliferate$ and $death$ to the alive state. Once cells move to the final state dead, they are eliminated from the system and from the simulation.

The transition connecting the state alive to the branch is triggered by the growth rate. In the state charts, the round squares represent the states and the arrows represent the transitions between the states. Arrows within states indicate the agent actions (or behaviours) and the final state is represented by a circle.

Our agents are stochastic and assume discrete time steps to execute their actions. This, however, does not restrict the dynamics of the models, as most of our agents state transitions are executed according to certain rates - this will go in parallel with steps execution, as defined in AnyLogic~\cite{AnyLogic:2010}. The rate triggered transition is used to model a stream of independent events (Poisson stream). In case more than one transition/interaction should occur at the same time, they are executed by AnyLogic in a discrete order in the same time-step. In the next section we apply the methodology to study our case studies and compare the outcomes.


==> RelatedWork.tex <==
\section*{Related Work}
\label{RelatedWork}

In this section we describe the literature concerned with the comparison between ODE and ABMS modelling for different simulation domains. We start our review by showing general work that has been carried out to assess the differences of both approaches. Subsequently, we focus on research concerned with the comparison of the strategies for immunological problems. We found that there is a scarcity of literature comparing the two approaches for immune simulations. Furthermore, to our knowledge there is no research contrasting the approaches for the immune system and cancer interactions.

Over the past years several authors have acknowledged that little work has been done to compare both methods. In one of the pioneer studies in this area, Scholl \cite{Scholl:2001a} gives an overview of ODE and ABMS, describes their areas of applicability and discusses the strengths and weaknesses of each approach. The author also tries to identify areas that could benefit from the use of both methodologies in multi-paradigm simulations and concludes that there is little literature concerned with the comparison of both methodologies and their cross studies. Pourdehnad {\it et al.} \cite{Pourdehnad:2002} compare the two
approaches conceptually by discussing the potential synergy between them to solve problems of teaching decision-making processes. The authors explore the conceptual frameworks for ODE modelling (using Systems Dynamics (SD)) and ABMS to model group learning and show the differences between the approaches in order to propose their use in a complementary way. They conclude that a lack of knowledge exists in applying multi-paradigm simulation that involves ODEs and ABMS. More recently, Stemate { \it et al.} \cite{Stemate:2007} also compare these modelling approaches and identify a list of likely opportunities for cross-fertilization. The authors see this list as a starting point for other researchers to take such synergistic views further.

Studies on this comparison for Operations Research were also conducted. For example, Schieritz \cite{Schieritz:2002} and  Scheritz {\it et al.}~\cite{Schieritz:2003} present a cross-study of SD (which is implemented using ODEs) and ABMS. They define their features and characteristics and contrast the two methods. In addition, they  suggest ideas of how to integrate both approaches. Continuing their studies, in \cite{Schieritz:2003b} the authors then describe an approach to combine ODEs and ABMS for solving supply chain management problems. Their results show that the combined SD/ABMS model does not produce the same outcomes as ODE model alone. To understand why these differences occur, the authors propose new tests as future work.

In an application in health care, Ramandad {\it et al.} \cite{Sterman:2008} compare the dynamics of a stochastic ABMS with those of the analogous deterministic compartment differential equation model for contagious disease spread. The authors convert the ABMS into an ODE model and examine the impact of individual heterogeneity and different network topologies. The deterministic model yields a single trajectory for each parameter set, while stochastic models yield a distribution of outcomes. Moreover, the ODE model and ABMS dynamics differ in several metrics relevant to public health. The responses of the models to policies can even differ when the base case behaviour is similar. Under some conditions, however, the differences in means are small, compared to variability caused by stochastic events, parameter uncertainty and model boundary.

An interesting philosophical analysis is conducted by Schieritz \cite{Schieritz:2004} analyses two arguments given in literature to explain the superiority of ABMS compared with ODEs: (1) ``{\it the inability of ODE models to explain emergent phenomena}'' and (2) ``{\it their flaw of not considering individual diversity}''. In analysing these arguments, the author considers different concepts involving simulation research in sociology. Moreover, the study identifies the theories of emergence that underlie the ODE and ABMS approaches. The author points out that ``{\it the agent-based approach models social phenomena by modelling individuals and interactions on a lower level, which makes it implicitly taking up an individualist position of emergence}; {\it ODEs, on the other hand, without explicitly referring to the concept of emergence, has a collectivist viewpoint of emergence, as it tends to model social phenomena on an aggregate system level}''. As a second part of the study, the author compares  ODEs and ABMS for modelling species competing for resources to analyse the effects of evolution on population dynamics. The conclusion is that when individual diversity is considered, it limits the applicability of the ODE model. However, it is shown that ``{\it a highly aggregate more ODE-like model of an evolutionary process displays similar results to the ABMS}''. This statement suggests that there is the need to investigate further the capabilities and equivalences of each approach.

Similarly, Lorenz ~\cite{Lorenz:2009} proposes that three aspects be compared and that this helps with the choice between ODE and ABMS: structure, behaviour and emergence. Structure is related to how the model is built. The structure of a model in ODE is static, whereas in ABMS it is dynamic. In ODE, all the elements, individuals and interactions of the simulation are developed in advance. In ABMS, on the other hand, agents are created or destroyed and interactions are defined through the course of the simulation run. The second aspect (behaviour) focuses on the central generators of behaviours in the model. For ODE the behaviour generators are feedback and accumulations, while for ABMS they are micro-macro-micro feedback and interaction of the systems elements. Both methodologies incorporate feedback. ABMS, however, has feedback in more than one level of modelling. The third aspect lies in their capacity to capture emergence, which differs between the two methodologies. In disagreement with\cite{Schieritz:2004} mentioned earlier, the author states that ABMS is capable of capturing emergence, while the one-level structure of ODE is insufficient in that respect.

In this work we discuss the merits of ODEs and ABMS for problems involving the interactions with the immune system and early-stage cancer that can benefit from either approach. To our knowledge (and as the gap in the literature shows) such a study has not been conducted before. The differences between ODEs and ABMS when applied to classes of problems belonging to different levels of abstraction are well established in the literature~\cite{Schieritz:2003}. However, we believe there is a range of problems that could benefit from being solved by both approaches. In addition, in many cases such as for example molecular and cellular biology, it is still not possible to use the full potential of ABMS as only the higher level of abstraction of the system is known.  Another reason to investigate problems that can interchangeably benefit from both approaches is that, as many real-world scenarios, such as biological systems, constantly gather new information, the corresponding simulations have to be updated frequently to suit new requirements. For some cases, in order to suit these demands, the replacement of the current simulation approach for new developments needs to be considered. Our case study investigation seeks to provide further understanding on these problems and fill some of the gaps existing in simulations for early-stage cancer research.

